A Note on Confluence in Typed Probabilistic Lambda Calculi

On the topic of probabilistic rewriting, there are several works studying both termination and confluence of different systems. While working with a lambda calculus modelling quantum computation, we found a system with probabilistic rewriting rules and strongly normalizing terms. We examine the effect of small modifications in probabilistic rewriting, affine variables, and strategies on the overall confluence in this strongly normalizing probabilistic calculus.

==> eptcsdata.tex <==
\providecommand{\firstpage}{18}
\providecommand{\publicationstatus}{Mauricio Ayala-Rinc\'on, Eduardo Bonelli (Eds.):
16th Logical \\ and Semantic Frameworks with Applications (LSFA 2021)\\
EPTCS 357, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.357.2}{10.4204/EPTCS.357.2}}
\pdfoutput=1

